Pushing the Limits of Vision-Language Models in Remote Sensing without Human Annotations

The prominence of generalized foundation models in vision-language integration has witnessed a surge, given their multifarious applications. Within the natural domain, the procurement of vision-language datasets to construct these foundation models is facilitated by their abundant availability and the ease of web crawling. Conversely, in the remote sensing domain, although vision-language datasets exist, their volume is suboptimal for constructing robust foundation models. This study introduces an approach to curate vision-language datasets by employing an image decoding machine learning model, negating the need for human-annotated labels. Utilizing this methodology, we amassed approximately 9.6 million vision-language paired datasets in VHR imagery. The resultant model outperformed counterparts that did not leverage publicly available vision-language datasets, particularly in downstream tasks such as zero-shot classification, semantic localization, and image-text retrieval. Moreover, in tasks exclusively employing vision encoders, such as linear probing and k-NN classification, our model demonstrated superior efficacy compared to those relying on domain-specific vision-language datasets.

==> Related_Work.tex <==
\subsection{Vision-Language Dataset in Natural Domain}

In the natural domain, there is already a vast amount of datasets available for building a vision-language foundation model. For example, the LAION-5B\cite{schuhmann2022laion} introduces a dataset comprising 5.85 billion CLIP\cite{radford2021learning}-filtered image-text pairs, which is 14 times larger than LAION-400M\cite{schuhmann2021laion}, the former largest publicly available image-text dataset globally. This dataset has been used to conduct a lot of research on vision-language foundation models\cite{fang2023eva, li2023scaling}, and it has shown great potential. In addition, various vision-language datasets such as CC12M\cite{changpinyo2021conceptual}, YFCC100M\cite{thomee2016yfcc100m} are making a great contribution to the research of vision-language foundation models in the natural domain.

\subsection{Vision-Language Dataset in Remote Sensing Domain}

In remote sensing, there are various vision-language datasets such as RSICD\cite{lu2017exploring}, UCM\cite{qu2016deep}, Sydney\cite{lu2017exploring} and RSITMD\cite{yuan2022exploring}. However, the amount of vision-language model is insufficient in order to build vision-language foundation model. Therefore, there are many achievements to address the lack of datasets without human assistance. The first is translating the datasets used for other purposes, such as object detection, instance segmentation and semantic segmentation, into vision-language sets. For example, the RemoteCLIP\cite{liu2023remoteclip} manipulate diverse datasets into vision-language sets. The second method is to create vision-language pairs using an image decoding machine learning model and filter them to create more accurate pairs, which is used in RS5M\cite{zhang2023rs5m}.












